Calibration and generalizability of probabilistic models on low-data chemical datasets with DIONYSUS

Deep learning models that leverage large datasets are often the state of the art for modelling molecular properties. When the datasets are smaller (< 2000 molecules), it is not clear that deep learning approaches are the right modelling tool. In this work we perform an extensive study of the calibration and generalizability of probabilistic machine learning models on small chemical datasets. Using different molecular representations and models, we analyse the quality of their predictions and uncertainties in a variety of tasks (binary, regression) and datasets. We also introduce two simulated experiments that evaluate their performance: (1) Bayesian optimization guided molecular design, (2) inference on out-of-distribution data via ablated cluster splits. We offer practical insights into model and feature choice for modelling small chemical datasets, a common scenario in new chemical experiments. We have packaged our analysis into the DIONYSUS repository, which is open sourced to aid in reproducibility and extension to new datasets.

==> insights.tex <==
\section{Insights} \label{sec:insights}

\begin{itemize}
    \item Gaussian Process + Mordred features are a solid modelling choice for small datasets. This combination faired well in all tasks and experiments. Model setup and optimization is relatively straightforward.
    \item Mordred features are quite robust independent of model choice. 
    \item NGBoost performs very well for much small datasets (<200 molecules), sometimes better than GPs.
    \item Deep Learning techniques suffer from bad performance for very low data regimes ($<300$ molecules). Their performance starts to become comparable to GPs after dataset sizes of 500 molecules. None the less, these techniques require careful more more work in terms of setup to properly regularize, select hyperparameters and stop model training (early stoping).
    \item Even thou purely predictive models ($\beta=0$) find hits faster, their model performance is much worse than any model with some exploratory component ($\beta>0$). We found that $beta=0.25$ tends to give .
\end{itemize}
